The Half-integral Erd\"os-P\'osa Property for Non-null Cycles

A Group Labeled Graph is a pair $(G,\Lambda)$ where $G$ is an oriented graph and $\Lambda$ is a mapping from the arcs of $G$ to elements of a group. A (not necessarily directed) cycle $C$ is called non-null if for any cyclic ordering of the arcs in $C$, the group element obtained by `adding' the labels on forward arcs and `subtracting' the labels on reverse arcs is not the identity element of the group. Non-null cycles in group labeled graphs generalize several well-known graph structures, including odd cycles. In this paper, we prove that non-null cycles on Group Labeled Graphs have the half-integral Erd\"os-P\'osa property. That is, there is a function $f:{\mathbb N}\to {\mathbb N}$ such that for any $k\in {\mathbb N}$, any group labeled graph $(G,\Lambda)$ has a set of $k$ non-null cycles such that each vertex of $G$ appears in at most two of these cycles or there is a set of at most $f(k)$ vertices that intersects every non-null cycle. Since it is known that non-null cycles do not have the integeral Erd\"os-P\'osa property in general, a half-integral Erd\"os-P\'osa result is the best one could hope for.

==> overview.tex <==
\section{Overview of the proof} Throughout the proof, we work with a fixed group. However, we do not assume anything regarding the size of the group or even that it is finite.
Our high level strategy, is the same as the standard approach used in \cite{,}. However, since we also need to take into account the fact that the group might be non-abelian.
We begin by arguing that the property holds on graphs of bounded treewidth. Following this,...

%Since our proof will be algorithmic, we will also end up proving Theorem \ref{}.

==> planar.tex <==
\section{{\erdosposa} property for non-null cycles in planar graphs}

In this section, we prove that the {\erdosposa} property holds for the family of non-null cycles on finite-group labeled \emph{planar} graphs.
